A Scalable Molecular Force Field Parameterization Method Based on Density Functional Theory and Quantum-Level Machine Learning

Fast and accurate molecular force field (FF) parameterization is still an unsolved problem. Accurate FFs are not generally available for all molecules, like novel druglike molecules. While methods based on quantum mechanics (QM) exist to parameterize them with better accuracy, they are computationally expensive and slow, which limits applicability to a small number of molecules. Here, we present an automated FF parameterization method which can utilize either DFT calculations or approximate QM energies produced by different neural network potentials (NNPs), to obtain improved parameters for molecules. We demonstrate that for the case of torchani-ANI-1x NNP, we can parameterize small molecules in a fraction of time compared with an equivalent parameterization using DFT QM calculations while producing more accurate parameters than FF (GAFF2). We expect our method to be of critical importance in computational structure-based drug discovery. The current version is available at PlayMolecule (www.playmolecule.org) and implemented in HTMD, allowing to parameterize molecules with different QM and NNP options.

==> zinc_table.tex <==
\clearpage
\begin{spacing}{1}
\begin{longtable}{ccccc}
\caption{Selected molecules from the ZINC dataset and their parameterization results.} \\
\toprule
ZINC ID & Number of atoms & Number of dihedral angles & Time (s) & MAE (kcal/mol) \\
\midrule
\endfirsthead
\toprule
ZINC ID & Number of atoms & Number of dihedral angles & Time (s) & MAE (kcal/mol) \\
\midrule
\endhead
\bottomrule
\endfoot
ZINC00331035 & 20 & 1 & 55 & 0.41 \\ 
ZINC00395657 & 22 & 1 & 40 & 0.02 \\ 
ZINC00410045 & 25 & 1 & 55 & 0.11 \\ 
ZINC01304634 & 12 & 1 & 32 & 0.14 \\ 
ZINC01393798 & 18 & 1 & 40 & 0.08 \\ 
ZINC01484813 & 22 & 1 & 46 & 0.11 \\ 
ZINC01612735 & 20 & 1 & 35 & 0.57 \\ 
ZINC01709106 & 33 & 1 & 80 & 0.07 \\ 
ZINC02541258 & 16 & 1 & 31 & 0.34 \\ 
ZINC04205172 & 26 & 1 & 48 & 0.17 \\ 
ZINC04955436 & 29 & 1 & 50 & 0.07 \\ 
ZINC04994129 & 30 & 1 & 58 & 0.07 \\ 
ZINC05019352 & 19 & 1 & 37 & 0.03 \\ 
ZINC05117701 & 15 & 1 & 33 & 0.15 \\ 
ZINC05766771 & 14 & 1 & 29 & 0.08 \\ 
ZINC11893845 & 21 & 1 & 55 & 0.12 \\ 
ZINC12647844 & 18 & 1 & 38 & 0.09 \\ 
ZINC12647864 & 22 & 1 & 32 & 0.02 \\ 
ZINC13538954 & 21 & 1 & 37 & 0.03 \\ 
ZINC13594926 & 23 & 1 & 48 & 0.27 \\ 
ZINC14684373 & 22 & 1 & 40 & 0.08 \\ 
ZINC17821249 & 22 & 1 & 43 & 0.03 \\ 
ZINC19505504 & 17 & 1 & 33 & 0.59 \\ 
ZINC19801863 & 27 & 1 & 51 & 0.42 \\ 
ZINC22005154 & 29 & 1 & 80 & 0.22 \\ 
ZINC24317785 & 25 & 1 & 47 & 0.13 \\ 
ZINC25494514 & 15 & 1 & 34 & 0.55 \\ 
ZINC25920511 & 19 & 1 & 34 & 0.08 \\ 
ZINC26895400 & 19 & 1 & 46 & 0.16 \\ 
ZINC28603460 & 23 & 1 & 40 & 0.03 \\ 
ZINC32189565 & 19 & 1 & 37 & 0.05 \\ 
ZINC33637874 & 26 & 1 & 56 & 0.08 \\ 
ZINC34161394 & 24 & 1 & 64 & 0.07 \\ 
ZINC36221926 & 29 & 1 & 59 & 0.05 \\ 
ZINC36448037 & 23 & 1 & 47 & 0.19 \\ 
ZINC36533565 & 18 & 1 & 65 & 0.03 \\ 
ZINC38350347 & 25 & 1 & 46 & 0.10 \\ 
ZINC38391215 & 27 & 1 & 45 & 0.04 \\ 
ZINC39071145 & 23 & 1 & 50 & 0.13 \\ 
ZINC39081391 & 25 & 1 & 59 & 0.71 \\ 
ZINC39114052 & 19 & 1 & 44 & 0.08 \\ 
ZINC39115025 & 24 & 1 & 45 & 0.05 \\ 
ZINC39136382 & 24 & 1 & 68 & 0.06 \\ 
ZINC39241537 & 25 & 1 & 48 & 0.05 \\ 
ZINC39262166 & 27 & 1 & 55 & 0.09 \\ 
ZINC39367473 & 23 & 1 & 45 & 0.03 \\ 
ZINC39368578 & 21 & 1 & 41 & 0.16 \\ 
ZINC39565242 & 19 & 1 & 41 & 0.04 \\ 
ZINC40448615 & 17 & 1 & 34 & 0.37 \\ 
ZINC41167351 & 23 & 1 & 49 & 0.03 \\ 
ZINC43193695 & 19 & 1 & 43 & 0.16 \\ 
ZINC43461290 & 17 & 1 & 32 & 0.05 \\ 
ZINC44062985 & 19 & 1 & 36 & 0.09 \\ 
ZINC49059545 & 21 & 1 & 42 & 0.05 \\ 
ZINC49806230 & 25 & 1 & 45 & 0.18 \\ 
ZINC51783681 & 28 & 1 & 76 & 0.48 \\ 
ZINC52886544 & 18 & 1 & 34 & 0.04 \\ 
ZINC54634189 & 18 & 1 & 35 & 0.02 \\ 
ZINC54822650 & 25 & 1 & 44 & 0.06 \\ 
ZINC58425246 & 26 & 1 & 49 & 0.28 \\ 
ZINC62605365 & 17 & 1 & 32 & 0.04 \\ 
ZINC62714202 & 22 & 1 & 78 & 0.02 \\ 
ZINC62715186 & 25 & 1 & 44 & 0.12 \\ 
ZINC67425272 & 19 & 1 & 37 & 0.04 \\ 
ZINC71496144 & 26 & 1 & 48 & 0.05 \\ 
ZINC71785324 & 18 & 1 & 32 & 0.04 \\ 
ZINC71785540 & 25 & 1 & 45 & 0.27 \\ 
ZINC71786905 & 27 & 1 & 45 & 0.10 \\ 
ZINC72230686 & 15 & 1 & 33 & 0.14 \\ 
ZINC72362052 & 30 & 1 & 61 & 0.53 \\ 
ZINC75541972 & 31 & 1 & 58 & 0.04 \\ 
ZINC76208564 & 27 & 1 & 63 & 0.18 \\ 
ZINC76575481 & 24 & 1 & 43 & 0.16 \\ 
ZINC76596617 & 28 & 1 & 48 & 0.06 \\ 
ZINC76596816 & 32 & 1 & 61 & 0.03 \\ 
ZINC76597950 & 27 & 1 & 58 & 0.02 \\ 
ZINC76598084 & 30 & 1 & 52 & 0.05 \\ 
ZINC76629135 & 33 & 1 & 60 & 0.04 \\ 
ZINC76629472 & 34 & 1 & 72 & 0.02 \\ 
ZINC82164281 & 25 & 1 & 55 & 0.18 \\ 
ZINC82396712 & 26 & 1 & 55 & 0.07 \\ 
ZINC82407024 & 26 & 1 & 49 & 0.09 \\ 
ZINC82474158 & 25 & 1 & 46 & 0.08 \\ 
ZINC82655499 & 29 & 1 & 55 & 0.05 \\ 
ZINC82869874 & 29 & 1 & 58 & 0.05 \\ 
ZINC82870517 & 28 & 1 & 61 & 0.07 \\ 
ZINC82871421 & 27 & 1 & 60 & 0.07 \\ 
ZINC82872552 & 26 & 1 & 61 & 0.13 \\ 
ZINC82875147 & 28 & 1 & 65 & 0.21 \\ 
ZINC83271269 & 32 & 1 & 73 & 0.04 \\ 
ZINC83273981 & 24 & 1 & 50 & 0.11 \\ 
ZINC85217577 & 21 & 1 & 37 & 0.06 \\ 
ZINC85345462 & 15 & 1 & 34 & 0.12 \\ 
ZINC95751936 & 17 & 1 & 41 & 0.38 \\ 
ZINC96865171 & 19 & 1 & 35 & 0.29 \\ 
ZINC00083985 & 19 & 2 & 39 & 0.86 \\ 
ZINC00339477 & 21 & 2 & 63 & 0.19 \\ 
ZINC01680841 & 22 & 2 & 56 & 0.14 \\ 
ZINC01690131 & 29 & 2 & 84 & 0.11 \\ 
ZINC01712450 & 27 & 2 & 95 & 0.17 \\ 
ZINC01736104 & 17 & 2 & 55 & 0.04 \\ 
ZINC01867185 & 22 & 2 & 59 & 0.05 \\ 
ZINC02504407 & 20 & 2 & 83 & 0.19 \\ 
ZINC02509813 & 29 & 2 & 129 & 0.13 \\ 
ZINC02578939 & 18 & 2 & 47 & 0.09 \\ 
ZINC04843852 & 25 & 2 & 67 & 0.03 \\ 
ZINC12380059 & 21 & 2 & 59 & 0.12 \\ 
ZINC12778463 & 27 & 2 & 85 & 0.13 \\ 
ZINC13545965 & 22 & 2 & 151 & 0.38 \\ 
ZINC19091690 & 24 & 2 & 70 & 0.13 \\ 
ZINC19424115 & 27 & 2 & 95 & 1.34 \\ 
ZINC19479577 & 28 & 2 & 89 & 0.09 \\ 
ZINC19735241 & 29 & 2 & 93 & 0.20 \\ 
ZINC20029292 & 14 & 2 & 44 & 0.05 \\ 
ZINC22004012 & 26 & 2 & 79 & 0.39 \\ 
ZINC23844576 & 27 & 2 & 82 & 0.14 \\ 
ZINC24332653 & 23 & 2 & 54 & 0.15 \\ 
ZINC26471409 & 17 & 2 & 58 & 0.07 \\ 
ZINC26506503 & 20 & 2 & 48 & 0.07 \\ 
ZINC32188564 & 22 & 2 & 68 & 0.20 \\ 
ZINC32210917 & 21 & 2 & 63 & 0.09 \\ 
ZINC33607615 & 27 & 2 & 80 & 0.23 \\ 
ZINC34247018 & 27 & 2 & 74 & 0.07 \\ 
ZINC36333661 & 20 & 2 & 58 & 0.08 \\ 
ZINC36947744 & 27 & 2 & 83 & 0.22 \\ 
ZINC39050950 & 20 & 2 & 85 & 0.08 \\ 
ZINC39051658 & 26 & 2 & 79 & 0.17 \\ 
ZINC39052236 & 20 & 2 & 53 & 0.08 \\ 
ZINC39081102 & 30 & 2 & 95 & 0.25 \\ 
ZINC39094769 & 20 & 2 & 61 & 0.18 \\ 
ZINC39111894 & 30 & 2 & 95 & 0.16 \\ 
ZINC39117983 & 20 & 2 & 50 & 0.11 \\ 
ZINC39612496 & 19 & 2 & 58 & 0.05 \\ 
ZINC41168102 & 26 & 2 & 76 & 0.05 \\ 
ZINC41168365 & 35 & 2 & 121 & 0.10 \\ 
ZINC44550797 & 22 & 2 & 85 & 0.15 \\ 
ZINC49469956 & 22 & 2 & 78 & 0.07 \\ 
ZINC49694165 & 33 & 2 & 107 & 0.12 \\ 
ZINC51890417 & 28 & 2 & 86 & 0.26 \\ 
ZINC51954366 & 31 & 2 & 105 & 0.16 \\ 
ZINC51954542 & 28 & 2 & 88 & 0.33 \\ 
ZINC52296411 & 29 & 2 & 117 & 0.17 \\ 
ZINC54404574 & 26 & 2 & 78 & 0.15 \\ 
ZINC57339690 & 24 & 2 & 77 & 0.51 \\ 
ZINC60713969 & 27 & 2 & 150 & 0.17 \\ 
ZINC62132670 & 23 & 2 & 66 & 0.22 \\ 
ZINC62772384 & 35 & 2 & 141 & 0.18 \\ 
ZINC71047790 & 19 & 2 & 54 & 0.80 \\ 
ZINC72275952 & 20 & 2 & 51 & 0.09 \\ 
ZINC74545630 & 23 & 2 & 62 & 0.58 \\ 
ZINC75556924 & 27 & 2 & 86 & 0.16 \\ 
ZINC75640625 & 28 & 2 & 95 & 0.09 \\ 
ZINC75845437 & 25 & 2 & 84 & 0.15 \\ 
ZINC76189012 & 24 & 2 & 46 & 0.20 \\ 
ZINC76570540 & 23 & 2 & 59 & 0.29 \\ 
ZINC76575551 & 25 & 2 & 70 & 0.08 \\ 
ZINC76577138 & 19 & 2 & 50 & 0.22 \\ 
ZINC76592067 & 33 & 2 & 115 & 0.14 \\ 
ZINC76599820 & 25 & 2 & 74 & 0.07 \\ 
ZINC76603537 & 31 & 2 & 106 & 0.09 \\ 
ZINC78725052 & 30 & 2 & 93 & 0.05 \\ 
ZINC82391337 & 26 & 2 & 113 & 0.23 \\ 
ZINC82399012 & 26 & 2 & 82 & 0.14 \\ 
ZINC82401944 & 27 & 2 & 88 & 0.11 \\ 
ZINC82406712 & 25 & 2 & 70 & 0.28 \\ 
ZINC82407479 & 21 & 2 & 84 & 0.12 \\ 
ZINC82408120 & 25 & 2 & 79 & 0.13 \\ 
ZINC82655557 & 23 & 2 & 62 & 0.07 \\ 
ZINC82748865 & 24 & 2 & 71 & 0.22 \\ 
ZINC82750442 & 27 & 2 & 72 & 0.06 \\ 
ZINC82822042 & 23 & 2 & 65 & 0.58 \\ 
ZINC82842034 & 22 & 2 & 62 & 0.15 \\ 
ZINC82842283 & 24 & 2 & 72 & 0.13 \\ 
ZINC82846609 & 20 & 2 & 64 & 0.05 \\ 
ZINC82851825 & 21 & 2 & 63 & 0.12 \\ 
ZINC82856022 & 31 & 2 & 118 & 0.25 \\ 
ZINC82868798 & 21 & 2 & 50 & 0.10 \\ 
ZINC82872831 & 30 & 2 & 132 & 0.13 \\ 
ZINC82879421 & 23 & 2 & 71 & 0.08 \\ 
ZINC83272882 & 28 & 2 & 83 & 0.16 \\ 
ZINC86862957 & 19 & 2 & 47 & 0.04 \\ 
ZINC90225792 & 28 & 2 & 80 & 0.09 \\ 
ZINC90411016 & 22 & 2 & 71 & 0.12 \\ 
ZINC95347751 & 23 & 2 & 61 & 0.08 \\ 
ZINC95773822 & 22 & 2 & 65 & 0.35 \\ 
ZINC95830253 & 24 & 2 & 58 & 0.09 \\ 
ZINC95883653 & 19 & 2 & 48 & 0.19 \\ 
ZINC96333791 & 29 & 2 & 107 & 0.11 \\ 
ZINC96863227 & 29 & 2 & 115 & 0.22 \\ 
ZINC00033566 & 24 & 3 & 89 & 0.19 \\ 
ZINC00039067 & 26 & 3 & 103 & 0.06 \\ 
ZINC00388053 & 20 & 3 & 67 & 0.26 \\ 
ZINC00394977 & 24 & 3 & 87 & 0.33 \\ 
ZINC01692335 & 25 & 3 & 123 & 0.13 \\ 
ZINC02528949 & 25 & 3 & 95 & 0.08 \\ 
ZINC02559282 & 24 & 3 & 105 & 0.09 \\ 
ZINC02562430 & 28 & 3 & 111 & 0.04 \\ 
ZINC02566074 & 20 & 3 & 67 & 0.05 \\ 
ZINC02571342 & 28 & 3 & 130 & 0.11 \\ 
ZINC04023436 & 24 & 3 & 112 & 0.28 \\ 
ZINC05177630 & 24 & 3 & 82 & 0.20 \\ 
ZINC05905888 & 22 & 3 & 91 & 0.10 \\ 
ZINC19091456 & 23 & 3 & 81 & 0.06 \\ 
ZINC19255175 & 19 & 3 & 72 & 0.06 \\ 
ZINC19255177 & 19 & 3 & 72 & 0.04 \\ 
ZINC19266016 & 30 & 3 & 141 & 0.09 \\ 
ZINC19511339 & 27 & 3 & 128 & 0.55 \\ 
ZINC19517445 & 27 & 3 & 113 & 0.16 \\ 
ZINC19702099 & 26 & 3 & 103 & 0.19 \\ 
ZINC19875495 & 23 & 3 & 89 & 0.10 \\ 
ZINC20177448 & 21 & 3 & 87 & 0.09 \\ 
ZINC21987634 & 24 & 3 & 88 & 0.03 \\ 
ZINC32629399 & 26 & 3 & 95 & 0.25 \\ 
ZINC33487059 & 26 & 3 & 83 & 0.16 \\ 
ZINC34343976 & 22 & 3 & 97 & 0.25 \\ 
ZINC34656726 & 31 & 3 & 160 & 0.08 \\ 
ZINC35679869 & 31 & 3 & 169 & 0.08 \\ 
ZINC35751511 & 29 & 3 & 128 & 0.19 \\ 
ZINC36240562 & 26 & 3 & 126 & 0.17 \\ 
ZINC36286966 & 26 & 3 & 127 & 0.22 \\ 
ZINC36327098 & 27 & 3 & 123 & 0.23 \\ 
ZINC36762089 & 19 & 3 & 80 & 0.05 \\ 
ZINC37184335 & 35 & 3 & 181 & 0.09 \\ 
ZINC38809898 & 24 & 3 & 102 & 1.12 \\ 
ZINC39094708 & 25 & 3 & 91 & 0.09 \\ 
ZINC39111370 & 25 & 3 & 103 & 0.09 \\ 
ZINC39295307 & 25 & 3 & 114 & 0.10 \\ 
ZINC40492339 & 39 & 3 & 238 & 0.14 \\ 
ZINC42769313 & 28 & 3 & 138 & 2.96 \\ 
ZINC42769723 & 23 & 3 & 84 & 0.12 \\ 
ZINC43802099 & 30 & 3 & 127 & 0.15 \\ 
ZINC44043507 & 28 & 3 & 141 & 0.15 \\ 
ZINC44095928 & 37 & 3 & 241 & 0.16 \\ 
ZINC45817562 & 30 & 3 & 146 & 0.12 \\ 
ZINC45956991 & 23 & 3 & 77 & 0.32 \\ 
ZINC51074877 & 26 & 3 & 99 & 0.07 \\ 
ZINC52211311 & 28 & 3 & 118 & 0.47 \\ 
ZINC54589392 & 27 & 3 & 117 & 0.14 \\ 
ZINC54599588 & 25 & 3 & 105 & 0.13 \\ 
ZINC54600294 & 27 & 3 & 112 & 0.52 \\ 
ZINC54789960 & 22 & 3 & 103 & 0.49 \\ 
ZINC54855306 & 22 & 3 & 66 & 0.03 \\ 
ZINC57763980 & 29 & 3 & 139 & 0.11 \\ 
ZINC58519123 & 29 & 3 & 163 & 0.59 \\ 
ZINC59290732 & 30 & 3 & 133 & 0.06 \\ 
ZINC61709339 & 25 & 3 & 95 & 0.16 \\ 
ZINC62112000 & 31 & 3 & 153 & 0.15 \\ 
ZINC62718582 & 23 & 3 & 85 & 0.06 \\ 
ZINC62719047 & 25 & 3 & 91 & 0.13 \\ 
ZINC64032871 & 24 & 3 & 107 & 0.13 \\ 
ZINC65731476 & 18 & 3 & 70 & 0.44 \\ 
ZINC66309437 & 19 & 3 & 63 & 0.07 \\ 
ZINC70957290 & 28 & 3 & 127 & 0.13 \\ 
ZINC71385466 & 32 & 3 & 178 & 0.16 \\ 
ZINC71795296 & 28 & 3 & 110 & 0.18 \\ 
ZINC72344410 & 29 & 3 & 136 & 0.40 \\ 
ZINC75840780 & 27 & 3 & 123 & 0.86 \\ 
ZINC76592117 & 33 & 3 & 144 & 0.17 \\ 
ZINC76602306 & 29 & 3 & 125 & 0.30 \\ 
ZINC76630513 & 33 & 3 & 173 & 0.07 \\ 
ZINC77265717 & 22 & 3 & 94 & 0.38 \\ 
ZINC79437394 & 31 & 3 & 149 & 0.26 \\ 
ZINC82392826 & 27 & 3 & 141 & 0.15 \\ 
ZINC82399017 & 27 & 3 & 143 & 0.17 \\ 
ZINC82399898 & 33 & 3 & 175 & 0.17 \\ 
ZINC82587630 & 26 & 3 & 145 & 0.22 \\ 
ZINC82837672 & 24 & 3 & 89 & 0.21 \\ 
ZINC82839550 & 28 & 3 & 105 & 0.12 \\ 
ZINC82844633 & 25 & 3 & 109 & 0.26 \\ 
ZINC82845494 & 28 & 3 & 135 & 0.35 \\ 
ZINC82847295 & 20 & 3 & 82 & 0.23 \\ 
ZINC82875093 & 28 & 3 & 68 & 0.48 \\ 
ZINC82875528 & 25 & 3 & 106 & 0.17 \\ 
ZINC82879711 & 28 & 3 & 120 & 0.28 \\ 
ZINC83273240 & 31 & 3 & 142 & 0.10 \\ 
ZINC83274046 & 29 & 3 & 118 & 0.29 \\ 
ZINC83274281 & 29 & 3 & 125 & 0.14 \\ 
ZINC83274339 & 29 & 3 & 133 & 2.42 \\ 
ZINC95723792 & 20 & 3 & 66 & 0.07 \\ 
ZINC95836673 & 28 & 3 & 132 & 0.19 \\ 
ZINC95883871 & 19 & 3 & 83 & 0.09 \\ 
ZINC00155965 & 23 & 4 & 143 & 0.27 \\ 
ZINC00391514 & 28 & 4 & 174 & 0.16 \\ 
ZINC01599030 & 24 & 4 & 116 & 0.21 \\ 
ZINC01617523 & 23 & 4 & 109 & 0.24 \\ 
ZINC01696266 & 24 & 4 & 137 & 0.09 \\ 
ZINC02037298 & 23 & 4 & 110 & 0.07 \\ 
ZINC02044667 & 24 & 4 & 105 & 0.16 \\ 
ZINC02245328 & 23 & 4 & 113 & 0.06 \\ 
ZINC02382702 & 27 & 4 & 128 & 0.09 \\ 
ZINC04244012 & 22 & 4 & 117 & 0.09 \\ 
ZINC05377596 & 24 & 4 & 159 & 0.25 \\ 
ZINC05666245 & 28 & 4 & 181 & 0.18 \\ 
ZINC05821980 & 33 & 4 & 192 & 0.12 \\ 
ZINC05984765 & 26 & 4 & 123 & 0.13 \\ 
ZINC06274137 & 31 & 4 & 158 & 0.10 \\ 
ZINC11631306 & 33 & 4 & 233 & 0.47 \\ 
ZINC12343549 & 31 & 4 & 172 & 0.04 \\ 
ZINC19402624 & 32 & 4 & 165 & 0.18 \\ 
ZINC19737135 & 39 & 4 & 253 & 0.18 \\ 
ZINC20475935 & 25 & 4 & 131 & 0.13 \\ 
ZINC20564712 & 24 & 4 & 120 & 0.25 \\ 
ZINC21955921 & 31 & 4 & 201 & 0.12 \\ 
ZINC26378814 & 26 & 4 & 155 & 0.24 \\ 
ZINC26510882 & 31 & 4 & 188 & 0.21 \\ 
ZINC31776768 & 21 & 4 & 105 & 0.13 \\ 
ZINC33953063 & 26 & 4 & 127 & 0.15 \\ 
ZINC35382256 & 25 & 4 & 139 & 0.45 \\ 
ZINC35390868 & 32 & 4 & 211 & 1.20 \\ 
ZINC36319813 & 32 & 4 & 221 & 0.17 \\ 
ZINC36770031 & 29 & 4 & 62 & 0.14 \\ 
ZINC36946857 & 31 & 4 & 177 & 1.12 \\ 
ZINC37467986 & 35 & 4 & 264 & 0.43 \\ 
ZINC37690099 & 32 & 4 & 183 & 0.06 \\ 
ZINC37690725 & 24 & 4 & 126 & 0.16 \\ 
ZINC37869967 & 23 & 4 & 130 & 0.42 \\ 
ZINC37996101 & 17 & 4 & 107 & 0.15 \\ 
ZINC38060876 & 30 & 4 & 184 & 0.16 \\ 
ZINC38642593 & 21 & 4 & 101 & 0.05 \\ 
ZINC39094967 & 25 & 4 & 129 & 0.13 \\ 
ZINC39113614 & 30 & 4 & 169 & 0.14 \\ 
ZINC39114906 & 24 & 4 & 114 & 0.07 \\ 
ZINC39136835 & 28 & 4 & 194 & 0.18 \\ 
ZINC39271935 & 25 & 4 & 115 & 0.20 \\ 
ZINC40543418 & 27 & 4 & 139 & 0.18 \\ 
ZINC41050802 & 30 & 4 & 143 & 0.13 \\ 
ZINC48914685 & 36 & 4 & 251 & 0.20 \\ 
ZINC50224436 & 28 & 4 & 156 & 0.54 \\ 
ZINC50464654 & 23 & 4 & 111 & 0.30 \\ 
ZINC52575431 & 28 & 4 & 185 & 0.23 \\ 
ZINC53096792 & 31 & 4 & 194 & 0.13 \\ 
ZINC53301968 & 26 & 4 & 113 & 0.08 \\ 
ZINC54456570 & 23 & 4 & 64 & 0.30 \\ 
ZINC54681419 & 28 & 4 & 67 & 0.40 \\ 
ZINC54697249 & 32 & 4 & 197 & 0.09 \\ 
ZINC61656802 & 28 & 4 & 130 & 0.12 \\ 
ZINC61818761 & 39 & 4 & 329 & 0.17 \\ 
ZINC61859660 & 27 & 4 & 74 & 0.48 \\ 
ZINC61932305 & 36 & 4 & 239 & 0.11 \\ 
ZINC71396781 & 25 & 4 & 124 & 0.09 \\ 
ZINC71396787 & 28 & 4 & 140 & 0.10 \\ 
ZINC71496588 & 35 & 4 & 198 & 0.13 \\ 
ZINC72194343 & 24 & 4 & 149 & 0.20 \\ 
ZINC75523122 & 20 & 4 & 89 & 0.11 \\ 
ZINC75853416 & 27 & 4 & 136 & 0.08 \\ 
ZINC76592557 & 31 & 4 & 173 & 0.05 \\ 
ZINC76599356 & 34 & 4 & 230 & 0.27 \\ 
ZINC76599744 & 27 & 4 & 135 & 0.33 \\ 
ZINC76630939 & 37 & 4 & 242 & 0.12 \\ 
ZINC76632847 & 23 & 4 & 70 & 0.36 \\ 
ZINC77262699 & 24 & 4 & 164 & 0.13 \\ 
ZINC82395728 & 29 & 4 & 177 & 0.50 \\ 
ZINC82401250 & 33 & 4 & 229 & 0.48 \\ 
ZINC82529503 & 27 & 4 & 145 & 0.26 \\ 
ZINC82632430 & 25 & 4 & 114 & 0.09 \\ 
ZINC82635655 & 34 & 4 & 212 & 0.30 \\ 
ZINC82636155 & 31 & 4 & 190 & 0.28 \\ 
ZINC82764613 & 29 & 4 & 149 & 0.05 \\ 
ZINC82856193 & 22 & 4 & 110 & 0.13 \\ 
ZINC82867937 & 34 & 4 & 218 & 0.10 \\ 
ZINC82868632 & 27 & 4 & 132 & 0.08 \\ 
ZINC82872495 & 26 & 4 & 134 & 0.13 \\ 
ZINC82873929 & 23 & 4 & 121 & 0.09 \\ 
ZINC82887135 & 32 & 4 & 213 & 0.16 \\ 
ZINC83255037 & 25 & 4 & 115 & 0.09 \\ 
ZINC83271062 & 22 & 4 & 110 & 0.14 \\ 
ZINC83271674 & 25 & 4 & 143 & 0.25 \\ 
ZINC83272041 & 18 & 4 & 86 & 0.93 \\ 
ZINC83272848 & 28 & 4 & 169 & 0.14 \\ 
ZINC83274598 & 22 & 4 & 136 & 0.23 \\ 
ZINC83339651 & 18 & 4 & 97 & 0.12 \\ 
ZINC95723452 & 22 & 4 & 99 & 0.13 \\ 
ZINC95883649 & 25 & 4 & 154 & 0.12 \\ 
ZINC96864669 & 34 & 4 & 234 & 0.17 \\ 
ZINC98095965 & 27 & 4 & 156 & 0.11 \\ 
ZINC01017016 & 25 & 5 & 162 & 0.09 \\ 
ZINC01602811 & 28 & 5 & 186 & 0.06 \\ 
ZINC01605992 & 36 & 5 & 213 & 0.07 \\ 
ZINC01634263 & 33 & 5 & 315 & 0.16 \\ 
ZINC01723600 & 27 & 5 & 182 & 0.12 \\ 
ZINC02004388 & 21 & 5 & 119 & 0.06 \\ 
ZINC02016150 & 26 & 5 & 152 & 0.33 \\ 
ZINC02047427 & 29 & 5 & 201 & 0.27 \\ 
ZINC02527113 & 31 & 5 & 191 & 0.44 \\ 
ZINC02528295 & 27 & 5 & 164 & 0.07 \\ 
ZINC02556034 & 19 & 5 & 107 & 0.02 \\ 
ZINC05007540 & 28 & 5 & 186 & 0.05 \\ 
ZINC05158496 & 21 & 5 & 156 & 0.23 \\ 
ZINC05528839 & 29 & 5 & 203 & 0.13 \\ 
ZINC05606218 & 20 & 5 & 132 & 0.17 \\ 
ZINC05768308 & 21 & 5 & 138 & 0.15 \\ 
ZINC09915897 & 21 & 5 & 112 & 0.13 \\ 
ZINC11889760 & 29 & 5 & 223 & 0.18 \\ 
ZINC13151262 & 34 & 5 & 252 & 0.24 \\ 
ZINC14505074 & 21 & 5 & 144 & 0.10 \\ 
ZINC19405550 & 31 & 5 & 227 & 0.11 \\ 
ZINC19485106 & 30 & 5 & 243 & 0.23 \\ 
ZINC19736889 & 27 & 5 & 157 & 0.08 \\ 
ZINC19736953 & 36 & 5 & 219 & 0.13 \\ 
ZINC19780628 & 32 & 5 & 243 & 0.07 \\ 
ZINC19875805 & 29 & 5 & 184 & 0.33 \\ 
ZINC20232064 & 29 & 5 & 181 & 0.48 \\ 
ZINC20382646 & 28 & 5 & 152 & 0.11 \\ 
ZINC21808532 & 27 & 5 & 185 & 0.32 \\ 
ZINC22123441 & 35 & 5 & 329 & 0.24 \\ 
ZINC26899082 & 24 & 5 & 131 & 0.50 \\ 
ZINC32153795 & 30 & 5 & 230 & 0.05 \\ 
ZINC34121635 & 24 & 5 & 186 & 0.16 \\ 
ZINC34259800 & 31 & 5 & 248 & 0.15 \\ 
ZINC34321053 & 30 & 5 & 221 & 0.12 \\ 
ZINC34355626 & 33 & 5 & 270 & 0.13 \\ 
ZINC34437590 & 25 & 5 & 174 & 0.08 \\ 
ZINC34598919 & 21 & 5 & 110 & 0.13 \\ 
ZINC34733048 & 28 & 5 & 173 & 0.08 \\ 
ZINC35603594 & 28 & 5 & 214 & 0.29 \\ 
ZINC36871023 & 25 & 5 & 157 & 0.09 \\ 
ZINC36962443 & 26 & 5 & 174 & 0.57 \\ 
ZINC37208344 & 33 & 5 & 265 & 0.11 \\ 
ZINC37224757 & 29 & 5 & 183 & 0.15 \\ 
ZINC37418594 & 27 & 5 & 197 & 0.25 \\ 
ZINC37471695 & 32 & 5 & 235 & 0.12 \\ 
ZINC37499759 & 29 & 5 & 254 & 0.32 \\ 
ZINC37688243 & 36 & 5 & 334 & 0.25 \\ 
ZINC37907116 & 28 & 5 & 194 & 0.42 \\ 
ZINC38005985 & 33 & 5 & 261 & 0.14 \\ 
ZINC38113237 & 30 & 5 & 213 & 0.24 \\ 
ZINC39087551 & 21 & 5 & 114 & 1.80 \\ 
ZINC40530300 & 22 & 5 & 130 & 0.20 \\ 
ZINC40925892 & 35 & 5 & 302 & 0.30 \\ 
ZINC42448679 & 25 & 5 & 101 & 0.32 \\ 
ZINC45930301 & 22 & 5 & 168 & 0.42 \\ 
ZINC49260408 & 34 & 5 & 280 & 0.12 \\ 
ZINC51816364 & 29 & 5 & 222 & 0.11 \\ 
ZINC51888442 & 32 & 5 & 277 & 0.93 \\ 
ZINC52144904 & 34 & 5 & 266 & 0.15 \\ 
ZINC52263358 & 30 & 5 & 88 & 0.15 \\ 
ZINC52574861 & 27 & 5 & 174 & 1.08 \\ 
ZINC53278585 & 30 & 5 & 173 & 0.13 \\ 
ZINC54072341 & 34 & 5 & 317 & 0.27 \\ 
ZINC54457587 & 25 & 5 & 90 & 1.77 \\ 
ZINC54555972 & 39 & 5 & 318 & 0.27 \\ 
ZINC55031724 & 35 & 5 & 286 & 0.08 \\ 
ZINC57935231 & 27 & 5 & 166 & 0.07 \\ 
ZINC61319170 & 31 & 5 & 267 & 0.34 \\ 
ZINC61701204 & 29 & 5 & 226 & 0.15 \\ 
ZINC61701207 & 29 & 5 & 234 & 0.11 \\ 
ZINC62128517 & 27 & 5 & 196 & 0.07 \\ 
ZINC62719180 & 27 & 5 & 163 & 0.16 \\ 
ZINC62761952 & 25 & 5 & 143 & 0.88 \\ 
ZINC68590868 & 39 & 5 & 399 & 0.40 \\ 
ZINC71499855 & 36 & 5 & 255 & 0.09 \\ 
ZINC71726779 & 24 & 5 & 156 & 0.25 \\ 
ZINC72259650 & 31 & 5 & 246 & 0.20 \\ 
ZINC75086287 & 29 & 5 & 210 & 0.25 \\ 
ZINC75542069 & 24 & 5 & 140 & 0.15 \\ 
ZINC75575848 & 22 & 5 & 128 & 0.52 \\ 
ZINC75577932 & 35 & 5 & 273 & 0.08 \\ 
ZINC76572585 & 25 & 5 & 138 & 0.10 \\ 
ZINC76579974 & 28 & 5 & 181 & 0.17 \\ 
ZINC76580872 & 38 & 5 & 339 & 0.33 \\ 
ZINC77268989 & 29 & 5 & 218 & 0.54 \\ 
ZINC78210623 & 26 & 5 & 179 & 0.43 \\ 
ZINC82402596 & 26 & 5 & 152 & 0.21 \\ 
ZINC82632765 & 28 & 5 & 254 & 0.08 \\ 
ZINC82633320 & 29 & 5 & 230 & 0.43 \\ 
ZINC82853158 & 30 & 5 & 215 & 0.12 \\ 
ZINC82855029 & 27 & 5 & 190 & 0.24 \\ 
ZINC82855038 & 27 & 5 & 189 & 0.19 \\ 
ZINC82855328 & 36 & 5 & 248 & 0.08 \\ 
ZINC83270020 & 27 & 5 & 172 & 0.12 \\ 
ZINC96862748 & 27 & 5 & 180 & 0.16 \\ 
ZINC00402956 & 30 & 6 & 250 & 0.23 \\ 
ZINC01698306 & 23 & 6 & 159 & 0.20 \\ 
ZINC01768433 & 29 & 6 & 198 & 0.14 \\ 
ZINC01852386 & 30 & 6 & 285 & 0.10 \\ 
ZINC02506664 & 34 & 6 & 280 & 0.05 \\ 
ZINC02556518 & 22 & 6 & 197 & 0.26 \\ 
ZINC02566751 & 26 & 6 & 176 & 0.05 \\ 
ZINC05335181 & 29 & 6 & 228 & 10.34 \\ 
ZINC05552274 & 26 & 6 & 179 & 0.09 \\ 
ZINC05712437 & 39 & 6 & 350 & 0.05 \\ 
ZINC06349948 & 27 & 6 & 201 & 0.48 \\ 
ZINC11978381 & 31 & 6 & 287 & 0.62 \\ 
ZINC12398082 & 31 & 6 & 231 & 0.06 \\ 
ZINC14690799 & 27 & 6 & 229 & 0.13 \\ 
ZINC17537002 & 25 & 6 & 191 & 0.47 \\ 
ZINC19431195 & 31 & 6 & 298 & 0.20 \\ 
ZINC19800904 & 34 & 6 & 252 & 0.07 \\ 
ZINC19834719 & 29 & 6 & 190 & 0.07 \\ 
ZINC19836601 & 24 & 6 & 172 & 0.20 \\ 
ZINC19912150 & 41 & 6 & 396 & 0.12 \\ 
ZINC19952852 & 29 & 6 & 255 & 0.17 \\ 
ZINC19967270 & 25 & 6 & 228 & 0.07 \\ 
ZINC20056761 & 33 & 6 & 303 & 0.16 \\ 
ZINC20182920 & 30 & 6 & 295 & 0.25 \\ 
ZINC20183031 & 28 & 6 & 257 & 0.32 \\ 
ZINC20434523 & 27 & 6 & 243 & 0.15 \\ 
ZINC20524171 & 39 & 6 & 485 & 0.25 \\ 
ZINC22000443 & 34 & 6 & 317 & 0.11 \\ 
ZINC32023514 & 29 & 6 & 264 & 0.15 \\ 
ZINC33640599 & 30 & 6 & 242 & 0.10 \\ 
ZINC34199433 & 24 & 6 & 102 & 0.18 \\ 
ZINC35321442 & 28 & 6 & 237 & 0.30 \\ 
ZINC35603389 & 33 & 6 & 297 & 0.17 \\ 
ZINC35604571 & 31 & 6 & 282 & 0.16 \\ 
ZINC35605863 & 25 & 6 & 203 & 0.23 \\ 
ZINC35747463 & 23 & 6 & 188 & 0.18 \\ 
ZINC36156313 & 33 & 6 & 200 & 0.04 \\ 
ZINC36747119 & 26 & 6 & 186 & 0.13 \\ 
ZINC36747447 & 29 & 6 & 275 & 0.15 \\ 
ZINC36778833 & 29 & 6 & 244 & 0.42 \\ 
ZINC37475613 & 27 & 6 & 233 & 0.34 \\ 
ZINC37475676 & 28 & 6 & 234 & 0.38 \\ 
ZINC37478710 & 34 & 6 & 368 & 0.17 \\ 
ZINC37629252 & 19 & 6 & 114 & 0.21 \\ 
ZINC37741332 & 38 & 6 & 335 & 0.25 \\ 
ZINC37996340 & 27 & 6 & 178 & 0.05 \\ 
ZINC38392070 & 30 & 6 & 214 & 0.10 \\ 
ZINC38804072 & 27 & 6 & 206 & 0.49 \\ 
ZINC39090331 & 35 & 6 & 324 & 0.30 \\ 
ZINC39393454 & 31 & 6 & 242 & 0.29 \\ 
ZINC40455650 & 27 & 6 & 232 & 0.19 \\ 
ZINC40494427 & 33 & 6 & 346 & 0.19 \\ 
ZINC40717088 & 34 & 6 & 304 & 0.18 \\ 
ZINC40920052 & 33 & 6 & 386 & 0.12 \\ 
ZINC40920648 & 28 & 6 & 256 & 0.73 \\ 
ZINC41053356 & 29 & 6 & 231 & 0.13 \\ 
ZINC41201305 & 29 & 6 & 193 & 0.05 \\ 
ZINC41201668 & 29 & 6 & 242 & 0.14 \\ 
ZINC41570612 & 25 & 6 & 198 & 0.15 \\ 
ZINC44068837 & 31 & 6 & 275 & 0.23 \\ 
ZINC44339503 & 28 & 6 & 220 & 0.62 \\ 
ZINC44339812 & 27 & 6 & 205 & 0.22 \\ 
ZINC49461587 & 24 & 6 & 201 & 0.29 \\ 
ZINC49805782 & 31 & 6 & 248 & 0.14 \\ 
ZINC50283805 & 28 & 6 & 255 & 0.12 \\ 
ZINC54071337 & 29 & 6 & 109 & 1.54 \\ 
ZINC54158211 & 28 & 6 & 272 & 0.12 \\ 
ZINC54374546 & 36 & 6 & 300 & 0.18 \\ 
ZINC54472716 & 33 & 6 & 339 & 0.14 \\ 
ZINC57933699 & 29 & 6 & 298 & 0.38 \\ 
ZINC57936222 & 31 & 6 & 266 & 0.58 \\ 
ZINC61680240 & 24 & 6 & 249 & 0.20 \\ 
ZINC61883103 & 34 & 6 & 358 & 0.30 \\ 
ZINC62454007 & 28 & 6 & 272 & 0.28 \\ 
ZINC66147895 & 32 & 6 & 264 & 0.31 \\ 
ZINC75437602 & 26 & 6 & 212 & 0.31 \\ 
ZINC75437613 & 23 & 6 & 162 & 0.24 \\ 
ZINC75518583 & 24 & 6 & 184 & 0.11 \\ 
ZINC75529580 & 21 & 6 & 142 & 0.24 \\ 
ZINC75543599 & 24 & 6 & 168 & 0.31 \\ 
ZINC76136001 & 28 & 6 & 202 & 0.12 \\ 
ZINC76580331 & 26 & 6 & 222 & 0.24 \\ 
ZINC76580393 & 36 & 6 & 376 & 0.76 \\ 
ZINC76581228 & 29 & 6 & 242 & 1.87 \\ 
ZINC77264963 & 33 & 6 & 306 & 0.20 \\ 
ZINC82587993 & 34 & 6 & 253 & 0.04 \\ 
ZINC82631675 & 26 & 6 & 212 & 1.41 \\ 
ZINC82632087 & 25 & 6 & 212 & 0.44 \\ 
ZINC82635596 & 30 & 6 & 226 & 0.18 \\ 
ZINC82855025 & 27 & 6 & 225 & 0.77 \\ 
ZINC82993183 & 31 & 6 & 240 & 0.08 \\ 
ZINC83144598 & 30 & 6 & 299 & 0.09 \\ 
ZINC83275557 & 31 & 6 & 250 & 0.30 \\ 
ZINC83340599 & 29 & 6 & 240 & 0.30 \\ 
ZINC83428444 & 27 & 6 & 208 & 0.42 \\ 
ZINC95080656 & 33 & 6 & 277 & 0.25 \\ 
ZINC96862862 & 25 & 6 & 201 & 0.25 \\ 
ZINC00404394 & 28 & 7 & 224 & 0.14 \\ 
ZINC01532560 & 25 & 7 & 189 & 0.14 \\ 
ZINC01605654 & 24 & 7 & 243 & 1.34 \\ 
ZINC01677121 & 20 & 7 & 135 & 0.08 \\ 
ZINC01683847 & 27 & 7 & 255 & 0.13 \\ 
ZINC01841432 & 22 & 7 & 188 & 0.19 \\ 
ZINC01845870 & 28 & 7 & 258 & 0.07 \\ 
ZINC01857612 & 23 & 7 & 213 & 0.25 \\ 
ZINC02011484 & 19 & 7 & 136 & 1.00 \\ 
ZINC02032391 & 25 & 7 & 186 & 0.07 \\ 
ZINC02042846 & 23 & 7 & 192 & 0.57 \\ 
ZINC02386044 & 25 & 7 & 171 & 0.12 \\ 
ZINC02530803 & 28 & 7 & 261 & 0.46 \\ 
ZINC02569673 & 33 & 7 & 375 & 0.31 \\ 
ZINC02572897 & 30 & 7 & 229 & 0.06 \\ 
ZINC02575089 & 35 & 7 & 357 & 0.17 \\ 
ZINC02582404 & 24 & 7 & 185 & 0.11 \\ 
ZINC03852391 & 26 & 7 & 199 & 0.10 \\ 
ZINC03977742 & 19 & 7 & 1008 & 0.24 \\ 
ZINC05463696 & 36 & 7 & 364 & 0.15 \\ 
ZINC05593213 & 36 & 7 & 412 & 0.44 \\ 
ZINC05820690 & 35 & 7 & 324 & 0.08 \\ 
ZINC05822037 & 35 & 7 & 357 & 0.23 \\ 
ZINC05871628 & 25 & 7 & 231 & 1.38 \\ 
ZINC06344280 & 27 & 7 & 235 & 0.15 \\ 
ZINC11959210 & 36 & 7 & 446 & 0.11 \\ 
ZINC14590537 & 21 & 7 & 154 & 0.63 \\ 
ZINC15204810 & 34 & 7 & 323 & 0.71 \\ 
ZINC15784534 & 36 & 7 & 389 & 0.21 \\ 
ZINC16575311 & 26 & 7 & 198 & 0.12 \\ 
ZINC19265292 & 33 & 7 & 333 & 0.13 \\ 
ZINC19508287 & 34 & 7 & 397 & 0.14 \\ 
ZINC20041786 & 38 & 7 & 412 & 0.15 \\ 
ZINC20041835 & 31 & 7 & 277 & 0.33 \\ 
ZINC20056519 & 33 & 7 & 287 & 0.08 \\ 
ZINC20083613 & 37 & 7 & 341 & 0.31 \\ 
ZINC20194887 & 36 & 7 & 455 & 0.21 \\ 
ZINC21999914 & 31 & 7 & 291 & 0.16 \\ 
ZINC22166504 & 27 & 7 & 245 & 0.34 \\ 
ZINC33432730 & 31 & 7 & 288 & 0.25 \\ 
ZINC33604901 & 33 & 7 & 347 & 0.07 \\ 
ZINC33841554 & 32 & 7 & 359 & 0.16 \\ 
ZINC35605222 & 25 & 7 & 229 & 0.60 \\ 
ZINC35795026 & 25 & 7 & 226 & 0.17 \\ 
ZINC36134700 & 28 & 7 & 304 & 2.11 \\ 
ZINC36420185 & 28 & 7 & 253 & 0.23 \\ 
ZINC37227198 & 30 & 7 & 241 & 0.07 \\ 
ZINC37476211 & 28 & 7 & 267 & 0.51 \\ 
ZINC37478733 & 29 & 7 & 310 & 0.38 \\ 
ZINC37478885 & 29 & 7 & 318 & 0.50 \\ 
ZINC37481584 & 31 & 7 & 341 & 0.36 \\ 
ZINC37625447 & 35 & 7 & 275 & 0.07 \\ 
ZINC37729933 & 35 & 7 & 378 & 0.28 \\ 
ZINC38004368 & 33 & 7 & 364 & 0.08 \\ 
ZINC38004623 & 38 & 7 & 411 & 0.18 \\ 
ZINC38116558 & 36 & 7 & 457 & 0.38 \\ 
ZINC38202311 & 24 & 7 & 272 & 0.59 \\ 
ZINC38665428 & 29 & 7 & 252 & 0.08 \\ 
ZINC39058322 & 20 & 7 & 161 & 0.30 \\ 
ZINC39058791 & 27 & 7 & 244 & 0.13 \\ 
ZINC39125816 & 31 & 7 & 298 & 0.25 \\ 
ZINC39135564 & 35 & 7 & 391 & 0.22 \\ 
ZINC40530234 & 23 & 7 & 223 & 1.98 \\ 
ZINC40920630 & 31 & 7 & 387 & 0.29 \\ 
ZINC42384208 & 25 & 7 & 202 & 0.19 \\ 
ZINC43199118 & 29 & 7 & 289 & 0.22 \\ 
ZINC43444176 & 34 & 7 & 298 & 0.05 \\ 
ZINC44475519 & 30 & 7 & 262 & 0.25 \\ 
ZINC44713484 & 28 & 7 & 242 & 0.13 \\ 
ZINC45072238 & 30 & 7 & 228 & 0.04 \\ 
ZINC49806138 & 37 & 7 & 368 & 0.22 \\ 
ZINC58267831 & 29 & 7 & 291 & 0.68 \\ 
ZINC58520607 & 30 & 7 & 248 & 0.13 \\ 
ZINC62719241 & 35 & 7 & 413 & 0.39 \\ 
ZINC68989336 & 30 & 7 & 302 & 0.06 \\ 
ZINC69553676 & 26 & 7 & 223 & 0.15 \\ 
ZINC71726829 & 27 & 7 & 265 & 0.31 \\ 
ZINC72235977 & 35 & 7 & 318 & 0.11 \\ 
ZINC74495643 & 24 & 7 & 223 & 0.57 \\ 
ZINC74525269 & 29 & 7 & 303 & 1.51 \\ 
ZINC74534655 & 31 & 7 & 364 & 0.94 \\ 
ZINC75523389 & 25 & 7 & 247 & 0.12 \\ 
ZINC75541385 & 24 & 7 & 232 & 0.09 \\ 
ZINC75546862 & 27 & 7 & 233 & 0.15 \\ 
ZINC75556649 & 27 & 7 & 226 & 0.66 \\ 
ZINC75565780 & 31 & 7 & 335 & 0.16 \\ 
ZINC76579848 & 30 & 7 & 276 & 0.51 \\ 
ZINC76580904 & 36 & 7 & 456 & 0.78 \\ 
ZINC76580907 & 36 & 7 & 482 & 0.33 \\ 
ZINC77271786 & 39 & 7 & 324 & 0.08 \\ 
ZINC82396987 & 31 & 7 & 263 & 0.38 \\ 
ZINC82399575 & 36 & 7 & 421 & 0.11 \\ 
ZINC82510413 & 32 & 7 & 348 & 0.46 \\ 
ZINC82635989 & 31 & 7 & 345 & 0.71 \\ 
ZINC83339713 & 28 & 7 & 285 & 0.23 \\ 
ZINC83341271 & 27 & 7 & 300 & 0.27 \\ 
ZINC85099936 & 36 & 7 & 462 & 0.17 \\ 
ZINC86050396 & 35 & 7 & 278 & 0.04 \\ 
ZINC87358147 & 36 & 7 & 408 & 0.17 \\ 
ZINC87358866 & 31 & 7 & 286 & 0.40 \\ 
ZINC01718585 & 23 & 8 & 241 & 0.14 \\ 
ZINC01846006 & 29 & 8 & 312 & 0.34 \\ 
ZINC01847857 & 26 & 8 & 196 & 0.09 \\ 
ZINC02509146 & 35 & 8 & 286 & 0.03 \\ 
ZINC02511794 & 31 & 8 & 340 & 0.12 \\ 
ZINC02527912 & 32 & 8 & 304 & 0.12 \\ 
ZINC02557989 & 34 & 8 & 386 & 0.70 \\ 
ZINC02565684 & 26 & 8 & 258 & 0.15 \\ 
ZINC02567644 & 27 & 8 & 158 & 0.43 \\ 
ZINC03647949 & 30 & 8 & 301 & 2.68 \\ 
ZINC04545871 & 31 & 8 & 392 & 0.36 \\ 
ZINC05452647 & 31 & 8 & 353 & 0.31 \\ 
ZINC05761895 & 31 & 8 & 255 & 0.16 \\ 
ZINC05820689 & 30 & 8 & 238 & 0.03 \\ 
ZINC05835776 & 32 & 8 & 350 & 0.15 \\ 
ZINC05973123 & 34 & 8 & 311 & 0.09 \\ 
ZINC12153814 & 30 & 8 & 360 & 0.22 \\ 
ZINC17328797 & 29 & 8 & 312 & 0.20 \\ 
ZINC19387869 & 34 & 8 & 494 & 0.08 \\ 
ZINC19396806 & 26 & 8 & 254 & 0.49 \\ 
ZINC19503633 & 33 & 8 & 357 & 1.06 \\ 
ZINC19506416 & 30 & 8 & 306 & 0.43 \\ 
ZINC19834742 & 35 & 8 & 315 & 0.10 \\ 
ZINC19870774 & 23 & 8 & 219 & 0.36 \\ 
ZINC20044280 & 36 & 8 & 352 & 0.07 \\ 
ZINC20047132 & 36 & 8 & 339 & 0.12 \\ 
ZINC20054100 & 35 & 8 & 491 & 0.82 \\ 
ZINC21950199 & 36 & 8 & 416 & 0.13 \\ 
ZINC21990226 & 30 & 8 & 352 & 0.09 \\ 
ZINC22034976 & 29 & 8 & 260 & 0.23 \\ 
ZINC26482801 & 33 & 8 & 290 & 0.11 \\ 
ZINC31477186 & 28 & 8 & 304 & 0.41 \\ 
ZINC32627172 & 34 & 8 & 451 & 0.43 \\ 
ZINC33611403 & 38 & 8 & 492 & 0.37 \\ 
ZINC35601630 & 39 & 8 & 560 & 0.13 \\ 
ZINC35602543 & 39 & 8 & 555 & 0.43 \\ 
ZINC36229973 & 28 & 8 & 305 & 0.14 \\ 
ZINC36667856 & 35 & 8 & 368 & 0.10 \\ 
ZINC37468703 & 31 & 8 & 387 & 0.17 \\ 
ZINC37480358 & 33 & 8 & 411 & 0.18 \\ 
ZINC38004393 & 38 & 8 & 450 & 0.08 \\ 
ZINC38004811 & 39 & 8 & 515 & 0.20 \\ 
ZINC38004835 & 41 & 8 & 544 & 0.23 \\ 
ZINC38024944 & 32 & 8 & 393 & 0.37 \\ 
ZINC38960067 & 32 & 8 & 260 & 0.04 \\ 
ZINC39058189 & 29 & 8 & 328 & 0.26 \\ 
ZINC39079902 & 27 & 8 & 302 & 1.65 \\ 
ZINC39126018 & 36 & 8 & 431 & 0.09 \\ 
ZINC39138988 & 33 & 8 & 410 & 3.26 \\ 
ZINC40774672 & 39 & 8 & 634 & 0.30 \\ 
ZINC41198894 & 31 & 8 & 313 & 0.11 \\ 
ZINC42453672 & 38 & 8 & 409 & 0.08 \\ 
ZINC43762849 & 31 & 8 & 375 & 0.34 \\ 
ZINC44339664 & 35 & 8 & 465 & 0.17 \\ 
ZINC45796435 & 24 & 8 & 254 & 0.48 \\ 
ZINC49804749 & 31 & 8 & 338 & 0.16 \\ 
ZINC49805081 & 38 & 8 & 398 & 0.07 \\ 
ZINC49805110 & 31 & 8 & 285 & 0.11 \\ 
ZINC49805135 & 38 & 8 & 340 & 0.07 \\ 
ZINC52378072 & 41 & 8 & 432 & 0.20 \\ 
ZINC52423201 & 38 & 8 & 525 & 0.31 \\ 
ZINC57218540 & 25 & 8 & 133 & 0.99 \\ 
ZINC59731889 & 29 & 8 & 347 & 0.31 \\ 
ZINC63170336 & 33 & 8 & 499 & 3.13 \\ 
ZINC66147934 & 33 & 8 & 428 & 0.22 \\ 
ZINC71715952 & 29 & 8 & 271 & 0.15 \\ 
ZINC71737238 & 32 & 8 & 406 & 0.23 \\ 
ZINC71786621 & 37 & 8 & 518 & 0.11 \\ 
ZINC71973519 & 26 & 8 & 257 & 0.27 \\ 
ZINC74495457 & 31 & 8 & 395 & 0.34 \\ 
ZINC74495876 & 32 & 8 & 388 & 0.50 \\ 
ZINC75545114 & 27 & 8 & 286 & 0.15 \\ 
ZINC75559515 & 25 & 8 & 246 & 0.33 \\ 
ZINC76579757 & 28 & 8 & 308 & 1.00 \\ 
ZINC76580176 & 33 & 8 & 451 & 1.06 \\ 
ZINC76580243 & 33 & 8 & 481 & 0.47 \\ 
ZINC76580254 & 33 & 8 & 336 & 0.87 \\ 
ZINC76580313 & 33 & 8 & 376 & 0.12 \\ 
ZINC76580867 & 27 & 8 & 303 & 0.51 \\ 
ZINC76580911 & 36 & 8 & 481 & 0.43 \\ 
ZINC76580929 & 36 & 8 & 544 & 0.90 \\ 
ZINC82391556 & 39 & 8 & 500 & 0.14 \\ 
ZINC82691234 & 35 & 8 & 367 & 0.82 \\ 
ZINC82691851 & 35 & 8 & 422 & 0.24 \\ 
ZINC83340196 & 31 & 8 & 374 & 0.06 \\ 
ZINC83340766 & 27 & 8 & 246 & 0.08 \\ 
ZINC83340911 & 30 & 8 & 266 & 0.12 \\ 
ZINC83341159 & 32 & 8 & 408 & 0.32 \\ 
ZINC90416356 & 41 & 8 & 454 & 0.04 \\ 
ZINC90469669 & 30 & 8 & 361 & 0.25 \\ 
ZINC95630366 & 26 & 8 & 299 & 0.52 \\ 
ZINC96034346 & 34 & 8 & 431 & 0.11 \\ 
ZINC96095586 & 41 & 8 & 434 & 0.07 \\ 
ZINC96334120 & 41 & 8 & 533 & 0.06 \\ 
ZINC96334293 & 41 & 8 & 615 & 0.07 \\ 
ZINC98088054 & 27 & 8 & 241 & 0.11 \\ 
ZINC98090896 & 32 & 8 & 270 & 0.40 \\ 
ZINC01529520 & 23 & 9 & 242 & 0.31 \\ 
ZINC01529776 & 30 & 9 & 434 & 0.58 \\ 
ZINC01566619 & 34 & 9 & 316 & 0.13 \\ 
ZINC01605928 & 33 & 9 & 257 & 0.10 \\ 
ZINC01640813 & 23 & 9 & 226 & 0.04 \\ 
ZINC01649339 & 30 & 9 & 517 & 1.03 \\ 
ZINC01684720 & 30 & 9 & 226 & 0.08 \\ 
ZINC01687484 & 36 & 9 & 359 & 0.06 \\ 
ZINC01688007 & 33 & 9 & 340 & 0.24 \\ 
ZINC01690951 & 27 & 9 & 302 & 0.68 \\ 
ZINC01698690 & 33 & 9 & 279 & 0.07 \\ 
ZINC01705962 & 29 & 9 & 360 & 0.21 \\ 
ZINC01730874 & 41 & 9 & 680 & 0.07 \\ 
ZINC01769346 & 29 & 9 & 273 & 0.20 \\ 
ZINC02020171 & 29 & 9 & 362 & 0.14 \\ 
ZINC02041822 & 28 & 9 & 170 & 1.71 \\ 
ZINC02170625 & 24 & 9 & 225 & 0.36 \\ 
ZINC02292293 & 33 & 9 & 344 & 0.48 \\ 
ZINC02386045 & 26 & 9 & 248 & 0.08 \\ 
ZINC02555771 & 32 & 9 & 390 & 0.09 \\ 
ZINC02560636 & 31 & 9 & 270 & 0.07 \\ 
ZINC02560655 & 29 & 9 & 256 & 0.09 \\ 
ZINC02567420 & 30 & 9 & 295 & 0.17 \\ 
ZINC02569623 & 28 & 9 & 249 & 0.04 \\ 
ZINC02578905 & 36 & 9 & 370 & 0.04 \\ 
ZINC02581404 & 30 & 9 & 385 & 0.16 \\ 
ZINC03872641 & 25 & 9 & 245 & 0.36 \\ 
ZINC04577736 & 24 & 9 & 258 & 0.80 \\ 
ZINC04782845 & 32 & 9 & 436 & 0.10 \\ 
ZINC05514153 & 32 & 9 & 342 & 0.15 \\ 
ZINC05553627 & 36 & 9 & 478 & 0.15 \\ 
ZINC05820434 & 33 & 9 & 364 & 0.09 \\ 
ZINC05822200 & 29 & 9 & 330 & 0.10 \\ 
ZINC06041116 & 31 & 9 & 312 & 0.13 \\ 
ZINC06041129 & 36 & 9 & 350 & 0.06 \\ 
ZINC14712784 & 35 & 9 & 400 & 0.08 \\ 
ZINC15120795 & 33 & 9 & 437 & 0.14 \\ 
ZINC19391151 & 40 & 9 & 687 & 0.26 \\ 
ZINC19397352 & 34 & 9 & 512 & 0.27 \\ 
ZINC20429565 & 32 & 9 & 294 & 0.12 \\ 
ZINC22010017 & 30 & 9 & 295 & 0.05 \\ 
ZINC25720288 & 31 & 9 & 347 & 0.12 \\ 
ZINC33432802 & 29 & 9 & 266 & 0.15 \\ 
ZINC34153516 & 39 & 9 & 512 & 0.10 \\ 
ZINC35602205 & 39 & 9 & 530 & 0.18 \\ 
ZINC36204157 & 33 & 9 & 317 & 0.06 \\ 
ZINC36667690 & 35 & 9 & 308 & 0.18 \\ 
ZINC36871387 & 34 & 9 & 410 & 0.22 \\ 
ZINC37480511 & 31 & 9 & 449 & 0.13 \\ 
ZINC37480621 & 34 & 9 & 460 & 0.13 \\ 
ZINC38600309 & 31 & 9 & 428 & 0.14 \\ 
ZINC39058005 & 26 & 9 & 297 & 0.15 \\ 
ZINC39058310 & 26 & 9 & 306 & 0.45 \\ 
ZINC39126313 & 32 & 9 & 438 & 0.19 \\ 
ZINC40216025 & 33 & 9 & 503 & 0.55 \\ 
ZINC40430766 & 36 & 9 & 516 & 0.19 \\ 
ZINC40832117 & 30 & 9 & 306 & 0.16 \\ 
ZINC40832349 & 36 & 9 & 427 & 0.11 \\ 
ZINC41043479 & 36 & 9 & 527 & 0.19 \\ 
ZINC42212153 & 31 & 9 & 316 & 0.21 \\ 
ZINC42691102 & 38 & 9 & 568 & 0.27 \\ 
ZINC43445244 & 32 & 9 & 454 & 0.14 \\ 
ZINC43445388 & 36 & 9 & 394 & 0.04 \\ 
ZINC49804751 & 31 & 9 & 293 & 0.05 \\ 
ZINC49805192 & 36 & 9 & 379 & 0.19 \\ 
ZINC52969548 & 39 & 9 & 561 & 0.29 \\ 
ZINC52973404 & 39 & 9 & 568 & 0.40 \\ 
ZINC52973405 & 39 & 9 & 551 & 0.17 \\ 
ZINC59245048 & 34 & 9 & 327 & 0.27 \\ 
ZINC66213836 & 31 & 9 & 312 & 0.14 \\ 
ZINC70671061 & 36 & 9 & 449 & 2.38 \\ 
ZINC71495641 & 33 & 9 & 326 & 0.09 \\ 
ZINC71495692 & 31 & 9 & 339 & 0.14 \\ 
ZINC71740404 & 30 & 9 & 394 & 0.23 \\ 
ZINC71741037 & 32 & 9 & 457 & 0.36 \\ 
ZINC71973565 & 29 & 9 & 311 & 0.15 \\ 
ZINC74320327 & 34 & 9 & 397 & 3.43 \\ 
ZINC74495593 & 34 & 9 & 437 & 0.13 \\ 
ZINC74495730 & 32 & 9 & 556 & 0.21 \\ 
ZINC75555356 & 25 & 9 & 155 & 0.24 \\ 
ZINC76580056 & 31 & 9 & 463 & 0.33 \\ 
ZINC76580076 & 31 & 9 & 365 & 1.06 \\ 
ZINC76580794 & 34 & 9 & 595 & 0.20 \\ 
ZINC76580825 & 34 & 9 & 546 & 0.11 \\ 
ZINC82080661 & 39 & 9 & 632 & 0.19 \\ 
ZINC82528424 & 34 & 9 & 509 & 0.19 \\ 
ZINC82691383 & 35 & 9 & 341 & 0.07 \\ 
ZINC82691667 & 35 & 9 & 332 & 0.08 \\ 
ZINC83340099 & 29 & 9 & 376 & 0.24 \\ 
ZINC83340100 & 29 & 9 & 359 & 0.23 \\ 
ZINC83340256 & 29 & 9 & 397 & 0.32 \\ 
ZINC83340275 & 29 & 9 & 346 & 0.26 \\ 
ZINC83341311 & 35 & 9 & 325 & 0.16 \\ 
ZINC83341384 & 34 & 9 & 450 & 0.07 \\ 
ZINC83422422 & 31 & 9 & 390 & 1.33 \\ 
ZINC86861065 & 26 & 9 & 233 & 0.18 \\ 
ZINC96326970 & 26 & 9 & 353 & 0.32 \\ 
ZINC96328217 & 36 & 9 & 370 & 0.06 \\ 
ZINC01529517 & 32 & 10 & 342 & 0.08 \\ 
ZINC01532698 & 36 & 10 & 609 & 0.42 \\ 
ZINC01610403 & 33 & 10 & 333 & 0.20 \\ 
ZINC01640802 & 26 & 10 & 311 & 0.12 \\ 
ZINC01640892 & 39 & 10 & 511 & 0.05 \\ 
ZINC01680237 & 31 & 10 & 308 & 0.03 \\ 
ZINC01685558 & 36 & 10 & 329 & 0.07 \\ 
ZINC01696789 & 37 & 10 & 397 & 0.33 \\ 
ZINC02009337 & 33 & 10 & 357 & 0.10 \\ 
ZINC02029799 & 39 & 10 & 391 & 0.05 \\ 
ZINC02037273 & 39 & 10 & 589 & 0.05 \\ 
ZINC02124171 & 33 & 10 & 361 & 0.18 \\ 
ZINC02516271 & 32 & 10 & 386 & 0.31 \\ 
ZINC02531050 & 32 & 10 & 315 & 0.08 \\ 
ZINC02575046 & 24 & 10 & 282 & 0.28 \\ 
ZINC03130416 & 36 & 10 & 481 & 0.10 \\ 
ZINC04095647 & 24 & 10 & 345 & 0.28 \\ 
ZINC04095649 & 24 & 10 & 297 & 0.15 \\ 
ZINC04533098 & 29 & 10 & 407 & 0.11 \\ 
ZINC05113046 & 30 & 10 & 327 & 0.08 \\ 
ZINC05131823 & 24 & 10 & 306 & 0.79 \\ 
ZINC05132035 & 24 & 10 & 333 & 0.70 \\ 
ZINC05132845 & 34 & 10 & 312 & 0.06 \\ 
ZINC05431007 & 34 & 10 & 440 & 0.12 \\ 
ZINC05467776 & 37 & 10 & 539 & 0.24 \\ 
ZINC05524264 & 39 & 10 & 559 & 0.16 \\ 
ZINC08580210 & 26 & 10 & 348 & 0.30 \\ 
ZINC11638642 & 34 & 10 & 360 & 0.16 \\ 
ZINC14825664 & 34 & 10 & 360 & 0.07 \\ 
ZINC19364631 & 34 & 10 & 382 & 0.04 \\ 
ZINC19441509 & 31 & 10 & 321 & 3.54 \\ 
ZINC19505256 & 34 & 10 & 394 & 0.10 \\ 
ZINC19517061 & 34 & 10 & 355 & 1.23 \\ 
ZINC19943572 & 34 & 10 & 408 & 0.07 \\ 
ZINC21996715 & 29 & 10 & 344 & 0.19 \\ 
ZINC21996719 & 29 & 10 & 365 & 0.28 \\ 
ZINC22034925 & 38 & 10 & 447 & 0.12 \\ 
ZINC22034929 & 38 & 10 & 494 & 0.09 \\ 
ZINC32164521 & 31 & 10 & 393 & 0.10 \\ 
ZINC33838178 & 26 & 10 & 340 & 0.15 \\ 
ZINC34500366 & 33 & 10 & 366 & 0.07 \\ 
ZINC34500369 & 33 & 10 & 341 & 0.06 \\ 
ZINC34518913 & 33 & 10 & 339 & 0.03 \\ 
ZINC34567089 & 29 & 10 & 291 & 0.06 \\ 
ZINC35075552 & 35 & 10 & 370 & 0.16 \\ 
ZINC35605909 & 34 & 10 & 356 & 3.61 \\ 
ZINC36984441 & 31 & 10 & 352 & 3.75 \\ 
ZINC37480549 & 34 & 10 & 488 & 0.29 \\ 
ZINC37480550 & 34 & 10 & 514 & 0.15 \\ 
ZINC37809434 & 34 & 10 & 491 & 0.26 \\ 
ZINC38652213 & 34 & 10 & 419 & 0.09 \\ 
ZINC39304027 & 34 & 10 & 403 & 0.11 \\ 
ZINC40830750 & 29 & 10 & 447 & 0.91 \\ 
ZINC40832405 & 36 & 10 & 559 & 0.29 \\ 
ZINC41620035 & 31 & 10 & 428 & 0.48 \\ 
ZINC43763483 & 30 & 10 & 417 & 0.39 \\ 
ZINC44135271 & 30 & 10 & 474 & 0.26 \\ 
ZINC44367542 & 33 & 10 & 324 & 0.03 \\ 
ZINC44709873 & 32 & 10 & 427 & 0.25 \\ 
ZINC45820074 & 34 & 10 & 354 & 0.06 \\ 
ZINC49580747 & 36 & 10 & 523 & 0.07 \\ 
ZINC49805249 & 34 & 10 & 354 & 0.04 \\ 
ZINC52599384 & 37 & 10 & 434 & 0.16 \\ 
ZINC59538622 & 31 & 10 & 373 & 0.06 \\ 
ZINC62719399 & 33 & 10 & 543 & 0.09 \\ 
ZINC65748465 & 32 & 10 & 472 & 0.17 \\ 
ZINC66068275 & 32 & 10 & 328 & 0.14 \\ 
ZINC70027719 & 32 & 10 & 543 & 1.00 \\ 
ZINC70626800 & 36 & 10 & 450 & 2.74 \\ 
ZINC71496861 & 36 & 10 & 410 & 0.11 \\ 
ZINC71496863 & 36 & 10 & 403 & 0.08 \\ 
ZINC71497060 & 34 & 10 & 383 & 0.10 \\ 
ZINC71741045 & 30 & 10 & 467 & 0.20 \\ 
ZINC71774182 & 29 & 10 & 338 & 0.13 \\ 
ZINC71973576 & 32 & 10 & 347 & 0.10 \\ 
ZINC74495437 & 34 & 10 & 550 & 0.42 \\ 
ZINC74496011 & 32 & 10 & 383 & 0.07 \\ 
ZINC75437623 & 39 & 10 & 375 & 0.04 \\ 
ZINC77285101 & 33 & 10 & 294 & 0.07 \\ 
ZINC82390885 & 32 & 10 & 400 & 0.07 \\ 
ZINC82390886 & 32 & 10 & 390 & 0.12 \\ 
ZINC83324678 & 33 & 10 & 410 & 0.24 \\ 
ZINC83324681 & 33 & 10 & 414 & 0.23 \\ 
ZINC83324688 & 31 & 10 & 194 & 5.06 \\ 
ZINC83340102 & 29 & 10 & 382 & 0.33 \\ 
ZINC83340192 & 31 & 10 & 354 & 0.10 \\ 
ZINC83340250 & 29 & 10 & 341 & 0.93 \\ 
ZINC83340251 & 29 & 10 & 364 & 0.96 \\ 
ZINC83340273 & 29 & 10 & 366 & 0.24 \\ 
ZINC83340328 & 27 & 10 & 343 & 1.13 \\ 
ZINC83341157 & 32 & 10 & 397 & 0.26 \\ 
ZINC83341314 & 36 & 10 & 453 & 0.63 \\ 
ZINC83341316 & 39 & 10 & 456 & 0.05 \\ 
ZINC83341375 & 34 & 10 & 436 & 0.08 \\ 
ZINC83341380 & 34 & 10 & 521 & 0.08 \\ 
ZINC83341383 & 34 & 10 & 453 & 0.06 \\ 
ZINC83341390 & 34 & 10 & 415 & 0.19 \\ 
ZINC87358502 & 39 & 10 & 487 & 0.35 \\ 
ZINC90225648 & 24 & 10 & 285 & 0.37 \\ 
ZINC96331822 & 26 & 10 & 376 & 0.18 \\ 
\end{longtable}
\end{spacing}

\clearpage
\begin{spacing}{1}
\begin{longtable}{ccccc}
\caption{Selected molecules from the ZINC dataset and their parameterization failures.} \\
\toprule
ZINC ID & Number of atoms & Number of dihedral angles & Failure \\
\midrule
\endfirsthead
\toprule
ZINC ID & Number of atoms & Number of dihedral angles & Failure \\
\midrule
\endhead
\bottomrule
\endfoot
ZINC47845034 & 22 & 1 & parameter fitting \\
ZINC52299020 & 34 & 1 & rotamer generation \\
ZINC77011161 & 21 & 1 & parameter fitting \\
ZINC82402743 & 21 & 1 & parameter fitting \\
ZINC82838277 & 21 & 1 & parameter fitting \\
ZINC19090386 & 15 & 2 & atom typing \\
ZINC19874139 & 25 & 2 & parameter fitting \\
ZINC45147273 & 18 & 2 & atom typing \\
ZINC70996057 & 27 & 2 & atom typing \\
ZINC83267280 & 17 & 2 & parameter fitting \\
ZINC95924468 & 26 & 2 & parameter fitting \\
ZINC12351911 & 26 & 3 & rotamer generation \\
ZINC37670806 & 27 & 3 & parameter fitting \\
ZINC38531460 & 23 & 3 & parameter fitting \\
ZINC52126090 & 31 & 3 & parameter fitting \\
ZINC73655766 & 36 & 3 & rotamer generation \\
ZINC75560676 & 15 & 3 & parameter fitting \\
ZINC77272295 & 28 & 3 & parameter fitting \\
ZINC98103322 & 26 & 3 & parameter fitting \\
ZINC02558026 & 19 & 4 & parameter fitting \\
ZINC36263209 & 20 & 4 & parameter fitting \\
ZINC40396945 & 27 & 4 & atom typing \\
ZINC54596551 & 28 & 4 & rotamer generation \\
ZINC82529487 & 29 & 4 & rotamer generation \\
ZINC82634081 & 28 & 4 & parameter fitting \\
ZINC37471775 & 28 & 5 & parameter fitting \\
ZINC54524091 & 28 & 5 & parameter fitting \\
ZINC61992181 & 34 & 5 & rotamer generation \\
ZINC76631273 & 23 & 5 & parameter fitting \\
ZINC13641439 & 31 & 6 & parameter fitting \\
ZINC36202439 & 27 & 6 & parameter fitting \\
ZINC40924436 & 26 & 6 & parameter fitting \\
ZINC13438090 & 26 & 8 & parameter fitting \\
ZINC39291440 & 34 & 8 & parameter fitting \\
ZINC52042525 & 35 & 8 & rotamer generation \\
ZINC03804508 & 31 & 9 & parameter fitting \\
ZINC83324690 & 28 & 9 & parameter fitting \\
\end{longtable}
\end{spacing}
